Data-Driven Estimation of Travel Latency Cost Functions via Inverse Optimization in Multi-Class Transportation Networks

We develop a method to estimate from data travel latency cost functions in multi-class transportation networks, which accommodate different types of vehicles with very different characteristics (e.g., cars and trucks). Leveraging our earlier work on inverse variational inequalities, we develop a data-driven approach to estimate the travel latency cost functions. Extensive numerical experiments using benchmark networks, ranging from moderate-sized to large-sized, demonstrate the effectiveness and efficiency of our approach.

==> mymacros_beamer.tex <==
% Equations ... 
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\newcommand{\benon}{\begin{equation*}}  
\newcommand{\bemuln}[1]{\begin{multline}\label{#1}}
\newcommand{\bemul}{\begin{multline*}}
\newcommand{\bee}{\begin{eqnarray*}}
\newcommand{\eee}{\end{eqnarray*}}
\newcommand{\been}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eeen}{\end{eqnarray}}
\newcommand{\began}[1]{\begin{gather}\label{#1}}
\newcommand{\bega}{\begin{gather*}}
\newcommand{\bealn}[1]{\begin{align}\label{#1}}
\newcommand{\beal}{\begin{align*}}
\newcommand{\bealatn}[2]{\begin{alignat}{#1}\label{#2}}
\newcommand{\bealat}{\begin{alignat*}}
\newcommand{\bexalatn}[1]{\begin{xalignat}\label{#1}}
\newcommand{\bexalat}{\begin{xalignat*}}


% Various...
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\pf}{\noindent \tcb{\bf Proof}:}
\newcommand{\disc}{\vskip 5 pt \noindent {\bf Discussion}\\}
\newcommand{\mot}{\vskip 5 pt \noindent {\bf Motivation}\\}
%\newcommand{\note}{\vskip 5 pt \noindent {\bf Note}\\}
\newcommand{\tsum}{\textstyle\sum}
\newcommand{\dsum}{\displaystyle\sum}


%Font commands
\newcommand{\mb}{\mathbf}
\newcommand{\bsy}{\boldsymbol}
\newcommand{\mn}{\mathnormal}
\newcommand{\mbb}{\mathbb}
\newcommand{\bosy}{\boldsymbol}


%Slides
\newcommand{\bs}{\begin{slide*}}
\newcommand{\es}{\end{slide*}}
\newcommand{\bsl}{\begin{slide}}
\newcommand{\esl}{\end{slide}}
\newcommand{\tits}[1]{\begin{center} \shadowbox{\large #1} \end{center}}
\newcommand{\bsf}[1]{\begin{frame}\frametitle{#1}}
\newcommand{\bsfl}[2]{\begin{frame}[label=#1]\frametitle{#2}}
\newcommand{\esf}{\end{frame}}

%Color
\DefineNamedColor{named}{BurntOrange}   {cmyk}{0,0.51,1,0}
\DefineNamedColor{named}{Red}           {cmyk}{0,1,1,0}
\DefineNamedColor{named}{Purple}        {cmyk}{0.45,0.86,0,0}
\DefineNamedColor{named}{NavyBlue}      {cmyk}{0.94,0.54,0,0}
\DefineNamedColor{named}{RoyalBlue}     {cmyk}{1,0.50,0,0}
\DefineNamedColor{named}{Blue}          {cmyk}{1,1,0,0}
\DefineNamedColor{named}{Cerulean}      {cmyk}{0.94,0.11,0,0}
\DefineNamedColor{named}{Cyan}          {cmyk}{1,0,0,0}
\DefineNamedColor{named}{Emerald}       {cmyk}{1,0,0.50,0}
\DefineNamedColor{named}{JungleGreen}   {cmyk}{0.99,0,0.52,0}
\DefineNamedColor{named}{SeaGreen}      {cmyk}{0.69,0,0.50,0}
\DefineNamedColor{named}{Green}         {cmyk}{1,0,1,0}
\DefineNamedColor{named}{ForestGreen}   {cmyk}{0.91,0,0.88,0.12}
\DefineNamedColor{named}{PineGreen}     {cmyk}{0.92,0,0.59,0.25}
\DefineNamedColor{named}{LimeGreen}     {cmyk}{0.50,0,1,0}
\DefineNamedColor{named}{YellowGreen}   {cmyk}{0.44,0,0.74,0}
\DefineNamedColor{named}{SpringGreen}   {cmyk}{0.26,0,0.76,0}
\DefineNamedColor{named}{OliveGreen}    {cmyk}{0.64,0,0.95,0.40}
\DefineNamedColor{named}{RawSienna}     {cmyk}{0,0.72,1,0.45}



\newcommand{\tc}{\textcolor}
\newcommand{\tcr}[1]{\tc{red}{#1}}
\newcommand{\tcb}[1]{\tc{blue}{#1}}
\newcommand{\tcgr}[1]{\tc{gray}{#1}}
\newcommand{\tcm}[1]{\tc{magenta}{#1}}
\newcommand{\tcg}[1]{\tc{green}{#1}}
\newcommand{\tcog}[1]{\textcolor[rgb]{0,0.55,0}{#1}}
\newcommand{\tcy}[1]{\textcolor[rgb]{0.95,0.95,0}{#1}}
\newcommand{\tcrb}[1]{\tc{RoyalBlue}{#1}}
\newcommand{\tcc}[1]{\tc{Cyan}{#1}}
\newcommand{\tcrs}[1]{\tc{RawSienna}{#1}}
\newcommand{\tcbo}[1]{\tc{BurntOrange}{#1}}
\newcommand{\tck}[1]{\tc{Black}{#1}}
\newcommand{\tcceru}[1]{\tc{Cerulean}{#1}}
\newcommand{\tcp}[1]{\textcolor[cmyk]{0.45,0.86,0,0}{#1}}







